Model Generation with LLMs: From Requirements to UML Sequence Diagrams

Complementing natural language (NL) requirements with graphical models can improve stakeholders' communication and provide directions for system design. However, creating models from requirements involves manual effort. The advent of generative large language models (LLMs), ChatGPT being a notable example, offers promising avenues for automated assistance in model generation. This paper investigates the capability of ChatGPT to generate a specific type of model, i.e., UML sequence diagrams, from NL requirements. We conduct a qualitative study in which we examine the sequence diagrams generated by ChatGPT for 28 requirements documents of various types and from different domains. Observations from the analysis of the generated diagrams have systematically been captured through evaluation logs, and categorized through thematic analysis. Our results indicate that, although the models generally conform to the standard and exhibit a reasonable level of understandability, their completeness and correctness with respect to the specified requirements often present challenges. This issue is particularly pronounced in the presence of requirements smells, such as ambiguity and inconsistency. The insights derived from this study can influence the practical utilization of LLMs in the RE process, and open the door to novel RE-specific prompting strategies targeting effective model generation.

==> sections/acknowledgement.tex <==
\sectopic{Acknowledgement. }
TODO
%This paper was supported by Central Legislative Service (SCL) -- Government of Luxembourg, the Luxembourg National Research Fund (FNR) under grants PUBLIC2-17/IS/11801776, and by NSERC of Canada under the Discovery and CRC programs.
% This paper was supported by Central Legislative Service (SCL) -- Government of Luxembourg, the European Research Council under the European Union's Horizon 2020 research
% and innovation programme (grant agreement No 694277), and NSERC of Canada under the Discovery and CRC programs.


==> sections/related-long.tex <==
\subsection{Related Work}\label{related-work} \hl{For sure it needs to be shortened, we keep this for a journal version.}
In the following we describe the related work on model generation and the application of LLMs in RE. We further discuss the research gaps which our work aims to address.  
\sectopic{Model Generation.} 
Model generation, also called model extraction, is a key task in NLP for RE. This consists of creating model abstractions---typically in a graphical form---from input requirements that can be expressed in different formats, e.g., ``shall'' requirements, use case specifications, or user stories. The systematic mapping study from Zhao \textit{et al.}~\cite{zhao2021natural}, which analyses studies in NLP for RE 1983 until 2019, counts 59 contributions concerning model generation, and the majority of the identified tools (26\%) target this task. Model generation can take different flavors~\cite{zhao2021natural}, from the generation of models to support requirements elicitation, analysis, and design~\cite{yue2015atoucan,chen2023use}, to the synthesis of feature models in a product-line engineering context~\cite{becan2016breathing}, to the generation of high-level models of early requirements or user stories to support project scoping~\cite{lucassen2017extracting}. In the following, we review the main reference works concerning UML model generation since this is the main focus of our contribution. For a comprehensive review on this topic, the reader should refer to \textit{Ahmed et al.}~\cite{ahmed2022automatic}.


The majority of the works focus on \textit{class diagram} generation, typically used for the representation of domain models, i.e., high-level abstraction of domain entities and relations thereof, which support early requirements analysis phases~\cite{saini2022automated}. One of the first contributions in this group is the CIRCE tool from Ambriola and Gervasi~\cite{ambriola2006systematic}. The tool uses NLP parsing rules to extract entities and relations to generate class diagrams, and it is also able to extract high-level data flow models. The proposal is showcased on a fictional yet representative example of a missile control system. 
Arora \textit{et al.}~\cite{arora2016extracting} proposes an approach that builds upon existing NLP rules from the literature, extended with novel ones exploiting dependency parsing. The approach is evaluated on a set of industrial requirements, and with a user study. An acknowledged limitation of the approach is the generation of irrelevant relationships, and the authors developed an active learning technique to discard these elements~\cite{arora2019active}. Saini \textit{et al.}~\cite{saini2022automated} present DoMoBOT, an interactive bot that not only generates domain models from problem descriptions but enables users to choose among different possible configurations. The approach combines rule-based NLP techniques with supervised machine learning, and it is evaluated on problem descriptions used as class exercises. 


Some of the existing contributions also address the generation of \textit{sequence diagrams} or similar behavioral representations such as message sequence charts (MSCs). Among them, the early contribution of Kof~\cite{kof2007scenarios} generates MSCs from scenario descriptions with a rule-based approach, which can also identify missing objects and actions in the original descriptions. The approach is evaluated on an industrial specification from the automotive domain. Yue \textit{et al.}~\cite{yue2015atoucan} present aToucan, a tool that extracts sequence diagrams---besides class and activity diagrams---from use case specifications expressed in a constrained natural language. The tool is based on a set of parsing and transformation rules and uses an intermediate representation to pass from the specifications to the final models. It is evaluated on two industrial case studies at Cisco Systems, Inc. More recently, Jahan \textit{et al.}~\cite{jahan2021generating} presents an approach that goes beyond previous contributions by accepting free text use case specifications instead of constrained natural language ones. Similarly to the other works, the approach is rule-based and evaluated on three simple problems.

%Other contributions focused on sequence diagrams and based on rules, but with limited evaluation, are, e.g., Thakur and Gupta~\cite{} and  

\sectopic{Large Language Models in RE.} 
LLMs are deep neural networks that use a transformer architecture and are pre-trained on large amounts of text via self-supervised learning to capture the statistical regularities and semantic knowledge in natural language~\cite{nguyen2023generative,min2023recent}. They are typically used as \textit{generative} models to produce human-like responses to natural language queries. LLMs can address several NLP tasks, such as question-answering, summarization, and translation. In our paper, we focus on question answering, a task consisting of generating the response to a question, normally referred to as \textit{prompt}. Well-known examples of LLMs for question answering are ChatGPT, Bing Chat (based on GPT4), Claude 2, Bard, and Vicuna (based on Llama). According to recent surveys on the usage of LLMs in software engineering~\cite{fan2023large,hou2023large}, the contributions concerning the usage of LLMs in RE are particularly scarce compared to other areas, such as testing, code generation, and program repair. In the following, we report some relevant examples. 

Jain \textit{et al.}~\cite{jain2023transformer} presents a set of experiments on the usage of different LLMs for requirements summarization from legal texts. They first generated summaries with the aid of GPT-3 and used them to fine-tune Pegasus, GPT-2, and other open-source models that do not require the disclosure of data, as in the case of GPT-3. Then, they evaluated the performance of these models on industrial datasets, showing that Pegasus outperforms the other options. Marczak \textit{et al.}~\cite{marczak2023using} use ChatGPT to generate user stories reflecting human values. The user stories are then used as creativity triggers in requirements elicitation sessions. The evaluation with focus groups shows that the generated user stories effectively inspire participants to identify value-relevant requirements. Rodriguez \textit{et al.}~\cite{rodriguez2023prompts} experiment with prompting strategies to support requirements traceability with the aid of Anthropic’s Claude instant model. Their exploratory evaluation with the CM1 dataset shows that small prompt modifications can lead to significant differences in model outputs. 

Some works also explore the potential of LLMs for model generation. Among them, Chen \textit{et al.}~\cite{chen2023use} evaluates the potential of GPT-4 for generating goal models using the textual grammar for the Goal-oriented Requirement Language (GRL) based on free-form natural NL descriptions of the problem context. Their experiments on four example cases show that incremental prompts can improve the results, and domain knowledge is highly needed to assess the plausible---yet frequently incorrect---output. Chen \textit{et al.}~\cite{chen2023automated} evaluates GPT-3.5 and GPT-4 for generating class diagrams based on NL descriptions. Their evaluation on a ground truth from an undergraduate course shows that the LLMs struggle to generate relationships between classes. Furthermore, they show that while few-shot approaches (i.e., adding examples to the prompts) can improve performance, chain-of-thought prompting (i.e., adding reasoning steps) leads to a performance decrease. Still on class diagram generation, Camára \textit{et al.}~\cite{camara2023assessment} perform an exploratory study using ChatGPT. They exercise the model with different sample problems and provide some lessons learned. The authors conclude that iterative prompting is needed to produce models of sufficient quality, and adherence to the standard in terms of construct semantics tends to be poor. Other studies in RE are generally dedicated to proposing pattern catalogs for specific problems, such as classification, traceability, and requirements elicitation~\cite{ronanki2023requirements,white2023chatgpt}. 

\sectopic{Research Gap} Most of the works on model generation in RE use rule-based approaches~\cite{ahmed2022automatic}. These typically require complex sets of heuristic rules, which are hardly maintainable and poorly adaptable to different contexts. One notable exception is the contribution by Saini \textit{et al.}~\cite{saini2022automated}, which enhances NLP rules with supervised machine learning for class diagram generation. However, this work does not use the most recent LLM-based technologies. The studies using LLMs in RE are scarce, but some focus on model generation. These are the exploratory studies by Camara \textit{et al.}~\cite{camara2023assessment} and Chen \textit{et al.}~\cite{chen2023automated}, targeting UML class diagram synthesis, and Chen et al.~\cite{chen2023use}, targeting goal models. However, these works do not focus on sequence diagrams and consider sample prompts rather than real-world specifications. Compared to previous work, our study is the first one to: (1) target UML sequence diagram generation using LLMs; (2) consider industrial requirements specifications as input; (3) consider different requirements types, i.e., ``shall'' requirements, user stories, and use case specifications.






